Stereo performance of SST-1M at different altitudes

The SST-1M telescopes are a pair of Imaging Atmospheric Cherenkov Telescopes (IACTs) that have been operating at the Ond\v{r}ejov Observatory (510 m a.s.l.) in the Czech Republic since 2022. Optimized for detecting gamma rays in the energy range 1-300 TeV, they are capable of performing both mono and stereo observations. Despite challenging atmospheric conditions, SST-1M has successfully detected several galactic and extragalactic gamma-ray sources with energies reaching up to 200 TeV during its ongoing commissioning. In this study, we analyze the performance of the SST-1M telescopes at different locations to assess the impact of altitude and relative telescope spacing on their physics performance. The low-altitude site at 510 m a.s.l. has already been investigated using both Monte Carlo simulations and real data. For comparison, we selected an intermediate-altitude site at 1420 m a.s.l. corresponding to Pampa Amarilla in Argentina and a high-altitude site at 4270 m a.s.l. corresponding to Hanle in India - both of which offer favorable astronomical conditions.

==> lit.tex <==
@article{Alispach_2025b,
    author = "Alispach, C. and others",
    title = "{Observation of the Crab Nebula with the Single-Mirror Small-Size Telescope stereoscopic system at low altitude}",
    eprint = "2506.01733",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    month = "6",
    year = "2025"
}

@ARTICLE{SST-1M,
       author = {{Alispach}, C. and {Araudo}, A. and {Balbo}, M. and {Beshley}, V. and {Biland}, A. and {Bla{\v{z}}ek}, J. and {Borkowski}, J. and {Bulik}, T. and {Cadoux}, F. and {Casanova}, S. and {Christov}, A. and {Chudoba}, J. and {Chytka}, L. and {D{\v{e}}di{\v{c}}}, P. and {della Volpe}, D. and {Favre}, Y. and {Garczarczyk}, M. and {Gibaud}, L. and {Gieras}, T. and {Hamal}, P. and {Heller}, M. and {Hrabovsk{\'y}}, M. and {Jane{\v{c}}ek}, P. and {Jel{\'\i}nek}, M. and {J{\'\i}lek}, V. and {Jury{\v{s}}ek}, J. and {Karas}, V. and {Lacave}, B. and {Lyard}, E. and {Mach}, E. and {Mand{\'a}t}, D. and {Marek}, W. and {Michal}, S. and {Micha{\l}owski}, J. and {Moderski}, R. and {Montaruli}, T. and {Muraczewski}, A. and {Muthyala}, S. and {M{\"u}ller}, A.~L. and {Nagai}, A. and {Nalewajski}, K. and {Neise}, D. and {Niemiec}, J. and {Niko{\l}ajuk}, M. and {Novotn{\'y}}, V. and {Ostrowski}, M. and {Palatka}, M. and {Pech}, M. and {Prouza}, M. and {Rajda}, P. and {Schovanek}, P. and {Seweryn}, K. and {Sliusar}, V. and {Stawarz}, {\L}. and {Sternberger}, R. and {Stodulska}, M. and {{\'S}wierblewski}, J. and {{\'S}wierk}, P. and {{\v{S}}trobl}, J. and {Tavernier}, T. and {Tr{\'a}vn{\'\i}{\v{c}}ek}, P. and {Troyano Pujadas}, I. and {V{\'\i}cha}, J. and {Vacula}, M. and {Walter}, R. and {Zi{\c{e}}tara}, K.},
        title = "{The SST-1M imaging atmospheric Cherenkov telescope for gamma-ray astrophysics}",
      journal = {\jcap},
     keywords = {gamma ray detectors, gamma ray experiments, cosmic ray experiments, cosmic rays detectors, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2025,
        month = feb,
       volume = {2025},
       number = {2},
          eid = {047},
        pages = {047},
          doi = {10.1088/1475-7516/2025/02/047},
archivePrefix = {arXiv},
       eprint = {2409.11310},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2025JCAP...02..047A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@techreport{1998cmcc.book.....H,
       author = {{Heck}, D. and {Knapp}, J. and {Capdevielle}, J.~N. and {Schatz}, G. and {Thouw}, T.},
        title = "{CORSIKA: a Monte Carlo code to simulate extensive air showers.}",
  institution = {Forschungszentrum Karlsruhe},
         type = {Report},
       number = {FZKA 6019},
         year = 1998
}

@article{BERNLOHR2008149,
author = {Konrad Bernlöhr},
title = {Simulation of imaging atmospheric Cherenkov telescopes with CORSIKA and sim_telarray},
journal = {Astroparticle Physics},
volume = {30},
number = {3},
pages = {149-158},
year = {2008},
issn = {0927-6505},
doi = {https://doi.org/10.1016/j.astropartphys.2008.07.009},
url = {https://www.sciencedirect.com/science/article/pii/S0927650508000972},
keywords = {Air showers, Imaging atmospheric Cherenkov technique, Gamma-ray astronomy},
}

@article{urqmd2,
    author = "Bleicher, M. and others",
    title = "{Relativistic hadron hadron collisions in the ultrarelativistic quantum molecular dynamics model}",
    eprint = "hep-ph/9909407",
    archivePrefix = "arXiv",
    doi = "10.1088/0954-3899/25/9/308",
    journal = "J. Phys. G",
    volume = "25",
    pages = "1859--1896",
    year = "1999"
}

@article{qgs,
      author         = "Ostapchenko, Sergey",
      title          = "{Monte Carlo treatment of hadronic interactions in
                        enhanced Pomeron scheme: I. QGSJET-II model}",
      journal        = "Phys. Rev. D",
      volume         = "83",
      year           = "2011",
      pages          = "014018",
      doi            = "10.1103/PhysRevD.83.014018",
      eprint         = "1010.1869",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1010.1869;%%"
}

@INPROCEEDINGS{modtran,
  author={Berk, A. and Conforti, P. and Kennett, R. and Perkins, T. and Hawes, F. and van den Bosch, J.},
  booktitle={2014 6th Workshop on Hyperspectral Image and Signal Processing: Evolution in Remote Sensing (WHISPERS)}, 
  title={MODTRAN® 6: A major upgrade of the MODTRAN® radiative transfer code}, 
  year={2014},
  volume={},
  number={},
  pages={1-4},
  keywords={Aerosols;Atmospheric modeling;Optical scattering;Software;Object oriented modeling;MODTRAN;remote sensing;hyperspectral;imaging;band model;radiative transfer;molecular transmittance},
  doi={10.1109/WHISPERS.2014.8077573}}



@software{sst1mpipe,
  author       = {Jurysek, Jakub and
                  Tavernier, Thomas and
                  Novotny, Vladimir and
                  Hamal, Petr and
                  Heller, Matthieu and
                  Blazek, Jiri and
                  Muraczewki, Adam and
                  Muthyala, Srija Reddy and
                  Alispach, Cyril and
                  Renier, Yves and
                  Coco, Victor},
  title        = {sst1mpipe: v0.7.3. 5 February 2025},
  month        = feb,
  year         = 2025,
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.14808846},
  url          = {https://doi.org/10.5281/zenodo.14808846},
}

@INPROCEEDINGS{jurysek_ICRC_proceeding,
       author = {{Jurysek}, J. and {Tavernier}, T. and {Novotn{\'y}}, V. and {Heller}, M. and {Mandat}, D. and {Pech}, M. and {Araudo}, A. and {Alispach}, C.~M. and {Beshley}, V. and {Blazek}, J. and {Borkowski}, J. and {Boula}, S. and {Bulik}, T. and {Cadoux}, F. and {Casanova}, S. and {Christov}, A. and {Chytka}, L. and {Favre}, Y. and {Gieras}, T. and {Hamal}, P. and {Hrabovsky}, M. and {Jelinek}, M. and {Karas}, V. and {Gibaud}, L. and {Lyard}, {\'E}. and {Mach}, E. and {Michal}, S. and {Michalowksi}, J. and {Moderski}, R. and {Montaruli}, T. and {Muthyala}, S.~R. and {Muraczewski}, A. and {Nalewajski}, K. and {Nagai}, A. and {Neise}, D. and {Niemiec}, J. and {Nikolajuk}, M. and {Palatka}, M. and {Prouza}, M. and {Rajda}, P. and {Schovanek}, P. and {Seweryn}, K. and {Sliusar}, V. and {Stawarz}, L. and {Strobl}, J. and {Swierk}, P. and {{\'S}wierblewski}, J. and {Travnicek}, P. and {Ostrowski}, M. and {Vicha}, J. and {Della Volpe}, D. and {Walter}, R. and {Marek}, W. and {Zagda{\'n}ski}, A. and {Zi{\c{e}}tara}, K.},
        title = "{Mono and stereo performance of the two SST-1M telescope prototypes}",
    booktitle = {38th International Cosmic Ray Conference},
         year = 2024,
        month = sep,
          eid = {592},
        pages = {592},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2024icrc.confE.592J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@software{ctapipe,
  author       = {Karl Kosack and
                  Jason Watson and
                  Maximilian Nöthe and
                  Jean Jacquemier and
                  Alison Mitchell and
                  Dominik Neise and
                  Christoph Deil and
                  Michele Peresano and
                  Samuel Timothy Spencer and
                  Lukas Nickel and
                  Raquel de los Reyes and
                  Franca Cassol and
                  Noah Biederbeck and
                  Kai Brügge and
                  Thomas Vuillaume and
                  Michele Mastropietro and
                  Jérémie Decock and
                  Abelardo Moralejo and
                  Wrijupan Bhattacharyya and
                  francesco visconti and
                  Jose Enrique Ruiz and
                  mgaug and
                  Ruben Lopez-Coto and
                  orelgueta and
                  Cyril Alispach and
                  Julien Lefaucheur and
                  Konstantin Pfrang and
                  Moritz Hütten and
                  thomasarmstrong and
                  Alice Donini},
  title        = {cta-observatory/ctapipe: v0.12.0},
  month        = nov,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {v0.12.0},
  doi          = {10.5281/zenodo.5720333},
  url          = {https://doi.org/10.5281/zenodo.5720333},
}


@article{crab_nebula_spectrum,
title = {The major upgrade of the MAGIC telescopes, Part II: A performance study using observations of the Crab Nebula},
journal = {Astroparticle Physics},
volume = {72},
pages = {76-94},
year = {2016},
issn = {0927-6505},
doi = {https://doi.org/10.1016/j.astropartphys.2015.02.005},
url = {https://www.sciencedirect.com/science/article/pii/S0927650515000316},
author = {J. Aleksić and S. Ansoldi and L.A. Antonelli and P. Antoranz and A. Babic and P. Bangale and M. Barceló and J.A. Barrio and J. {Becerra González} and W. Bednarek and E. Bernardini and B. Biasuzzi and A. Biland and M. Bitossi and O. Blanch and S. Bonnefoy and G. Bonnoli and F. Borracci and T. Bretz and E. Carmona and A. Carosi and R. Cecchi and P. Colin and E. Colombo and J.L. Contreras and D. Corti and J. Cortina and S. Covino and P. {Da Vela} and F. Dazzi and A. {De Angelis} and G. {De Caneva} and B. {De Lotto} and E. {de Oña Wilhelmi} and C. {Delgado Mendez} and A. Dettlaff and D. {Dominis Prester} and D. Dorner and M. Doro and S. Einecke and D. Eisenacher and D. Elsaesser and D. Fidalgo and D. Fink and M.V. Fonseca and L. Font and K. Frantzen and C. Fruck and D. Galindo and R.J. {García López} and M. Garczarczyk and D. {Garrido Terrats} and M. Gaug and G. Giavitto and N. Godinović and A. {González Muñoz} and S.R. Gozzini and W. Haberer and D. Hadasch and Y. Hanabata and M. Hayashida and J. Herrera and D. Hildebrand and J. Hose and D. Hrupec and W. Idec and J.M. Illa and V. Kadenius and H. Kellermann and M.L. Knoetig and K. Kodani and Y. Konno and J. Krause and H. Kubo and J. Kushida and A. {La Barbera} and D. Lelas and J.L. Lemus and N. Lewandowska and E. Lindfors and S. Lombardi and F. Longo and M. López and R. López-Coto and A. López-Oramas and A. Lorca and E. Lorenz and I. Lozano and M. Makariev and K. Mallot and G. Maneva and N. Mankuzhiyil and K. Mannheim and L. Maraschi and B. Marcote and M. Mariotti and M. Martínez and D. Mazin and U. Menzel and J.M. Miranda and R. Mirzoyan and A. Moralejo and P. Munar-Adrover and D. Nakajima and M. Negrello and V. Neustroev and A. Niedzwiecki and K. Nilsson and K. Nishijima and K. Noda and R. Orito and A. Overkemping and S. Paiano and M. Palatiello and D. Paneque and R. Paoletti and J.M. Paredes and X. Paredes-Fortuny and M. Persic and J. Poutanen and P.G. {Prada Moroni} and E. Prandini and I. Puljak and R. Reinthal and W. Rhode and M. Ribó and J. Rico and J. {Rodriguez Garcia} and S. Rügamer and T. Saito and K. Saito and K. Satalecka and V. Scalzotto and V. Scapin and C. Schultz and J. Schlammer and S. Schmidl and T. Schweizer and S.N. Shore and A. Sillanpää and J. Sitarek and I. Snidaric and D. Sobczynska and F. Spanier and A. Stamerra and T. Steinbring and J. Storz and M. Strzys and L. Takalo and H. Takami and F. Tavecchio and L.A. Tejedor and P. Temnikov and T. Terzić and D. Tescaro and M. Teshima and J. Thaele and O. Tibolla and D.F. Torres and T. Toyama and A. Treves and P. Vogler and H. Wetteskind and M. Will and R. Zanin},
keywords = {Gamma-ray astronomy, Cherenkov telescopes, Crab Nebula},
abstract = {MAGIC is a system of two Imaging Atmospheric Cherenkov Telescopes located in the Canary island of La Palma, Spain. During summer 2011 and 2012 it underwent a series of upgrades, involving the exchange of the MAGIC-I camera and its trigger system, as well as the upgrade of the readout system of both telescopes. We use observations of the Crab Nebula taken at low and medium zenith angles to assess the key performance parameters of the MAGIC stereo system. For low zenith angle observations, the standard trigger threshold of the MAGIC telescopes is ∼ 50 GeV. The integral sensitivity for point-like sources with Crab Nebula-like spectrum above 220GeV is (0.66 ± 0.03)% of Crab Nebula flux in 50h of observations. The angular resolution, defined as the σ of a 2-dimensional Gaussian distribution, at those energies is ≲ 0.07°, while the energy resolution is 16%. We also re-evaluate the effect of the systematic uncertainty on the data taken with the MAGIC telescopes after the upgrade. We estimate that the systematic uncertainties can be divided in the following components: < 15% in energy scale, 11%–18% in flux normalization and ± 0.15 for the energy spectrum power-law slope.}
}


@article{proton_spectrum,
  title = {Measurement of the cosmic $p+\mathrm{He}$ energy spectrum from 50 GeV to 0.5 PeV with the DAMPE space mission},
  author = {Alemanno, F. and Altomare, C. and An, Q. and Azzarello, P. and Barbato, F. C. T. and Bernardini, P. and Bi, X. J. and Cagnoli, I. and Cai, M. S. and Casilli, E. and Catanzani, E. and Chang, J. and Chen, D. Y. and Chen, J. L. and Chen, Z. F. and Coppin, P. and Cui, M. Y. and Cui, T. S. and Cui, Y. X. and Dai, H. T. and De Benedittis, A. and De Mitri, I. and de Palma, F. and Deliyergiyev, M. and Di Giovanni, A. and Di Santo, M. and Ding, Q. and Dong, T. K. and Dong, Z. X. and Donvito, G. and Droz, D. and Duan, J. L. and Duan, K. K. and Fan, R. R. and Fan, Y. Z. and Fang, F. and Fang, K. and Feng, C. Q. and Feng, L. and Alonso, M. Fernandez and Frieden, J. M. and Fusco, P. and Gao, M. and Gargano, F. and Gong, K. and Gong, Y. Z. and Guo, D. Y. and Guo, J. H. and Han, S. X. and Hu, Y. M. and Huang, G. S. and Huang, X. Y. and Huang, Y. Y. and Ionica, M. and Jiang, L. Y. and Jiang, Y. Z. and Jiang, W. and Kong, J. and Kotenko, A. and Kyratzis, D. and Lei, S. J. and Li, W. H. and Li, W. L. and Li, X. and Li, X. Q. and Liang, Y. M. and Liu, C. M. and Liu, H. and Liu, J. and Liu, S. B. and Liu, Y. and Loparco, F. and Luo, C. N. and Ma, M. and Ma, P. X. and Ma, T. and Ma, X. Y. and Marsella, G. and Mazziotta, M. N. and Mo, D. and Salinas, M. Muoz and Niu, X. Y. and Pan, X. and Parenti, A. and Peng, W. X. and Peng, X. Y. and Perrina, C. and Putti-Garcia, E. and Qiao, R. and Rao, J. N. and Ruina, A. and Shangguan, Z. and Shen, W. H. and Shen, Z. Q. and Shen, Z. T. and Silveri, L. and Song, J. X. and Stolpovskiy, M. and Su, H. and Su, M. and Sun, H. R. and Sun, Z. Y. and Surdo, A. and Teng, X. J. and Tykhonov, A. and Wang, J. Z. and Wang, L. G. and Wang, S. and Wang, S. X. and Wang, X. L. and Wang, Y. and Wang, Y. F. and Wang, Y. Z. and Wang, Z. M. and Wei, D. M. and Wei, J. J. and Wei, Y. F. and Wu, D. and Wu, J. and Wu, L. B. and Wu, S. S. and Wu, X. and Xia, Z. Q. and Xu, H. T. and Xu, J. and Xu, Z. H. and Xu, Z. L. and Xu, E. H. and Xu, Z. Z. and Xue, G. F. and Yang, H. B. and Yang, P. and Yang, Y. Q. and Yao, H. J. and Yu, Y. H. and Yuan, G. W. and Yuan, Q. and Yue, C. and Zang, J. J. and Zhang, S. X. and Zhang, W. Z. and Zhang, Yan and Zhang, Yi and Zhang, Y. J. and Zhang, Y. L. and Zhang, Y. P. and Zhang, Y. Q. and Zhang, Z. and Zhang, Z. Y. and Zhao, C. and Zhao, H. Y. and Zhao, X. F. and Zhou, C. Y. and Zhu, Y.},
  collaboration = {DAMPE Collaboration},
  journal = {Phys. Rev. D},
  volume = {109},
  issue = {12},
  pages = {L121101},
  numpages = {8},
  year = {2024},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.109.L121101},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.109.L121101}
}


@article{cta_site_selection,
title = {Monte Carlo performance studies for the site selection of the Cherenkov Telescope Array},
journal = {Astroparticle Physics},
volume = {93},
pages = {76-85},
year = {2017},
issn = {0927-6505},
doi = {https://doi.org/10.1016/j.astropartphys.2017.05.001},
url = {https://www.sciencedirect.com/science/article/pii/S0927650517300087},
author = {T. Hassan and L. Arrabito and K. Bernlöhr and J. Bregeon and J. Cortina and P. Cumani and F. {Di Pierro} and D. Falceta-Goncalves and R.G. Lang and J. Hinton and T. Jogler and G. Maier and A. Moralejo and A. Morselli and C.J. {Todero Peixoto} and M. Wood},
keywords = {Monte Carlo simulations, Cherenkov Telescopes, IACT technique, Gamma rays, Cosmic rays},
abstract = {The Cherenkov Telescope Array (CTA) represents the next generation of ground-based instruments for very-high-energy (VHE) gamma-ray astronomy, aimed at improving on the sensitivity of current-generation experiments by an order of magnitude and providing coverage over four decades of energy. The current CTA design consists of two arrays of tens of imaging atmospheric Cherenkov Telescopes, comprising Small, Medium and Large-Sized Telescopes, with one array located in each of the Northern and Southern Hemispheres. To study the effect of the site choice on the overall CTA performance and support the site evaluation process, detailed Monte Carlo simulations have been performed. These results show the impact of different site-related attributes such as altitude, night-sky background and local geomagnetic field on CTA performance for the observation of VHE gamma rays.}
}

@article{cta_layout_config,
title = {Monte Carlo studies for the optimisation of the Cherenkov Telescope Array layout},
journal = {Astroparticle Physics},
volume = {111},
pages = {35-53},
year = {2019},
issn = {0927-6505},
doi = {https://doi.org/10.1016/j.astropartphys.2019.04.001},
url = {https://www.sciencedirect.com/science/article/pii/S0927650519300234},
author = {A. Acharyya and I. Agudo and E.O. Angüner and R. Alfaro and J. Alfaro and C. Alispach and R. Aloisio and R. {Alves Batista} and J.-P. Amans and L. Amati and E. Amato and G. Ambrosi and L.A. Antonelli and C. Aramo and T. Armstrong and F. Arqueros and L. Arrabito and K. Asano and H. Ashkar and C. Balazs and M. Balbo and B. Balmaverde and P. Barai and A. Barbano and M. Barkov and U. {Barres de Almeida} and J.A. Barrio and D. Bastieri and J. {Becerra González} and J. {Becker Tjus} and L. Bellizzi and W. Benbow and E. Bernardini and M.I. Bernardos and K. Bernlöhr and A. Berti and M. Berton and B. Bertucci and V. Beshley and B. Biasuzzi and C. Bigongiari and R. Bird and E. Bissaldi and J. Biteau and O. Blanch and J. Blazek and C. Boisson and G. Bonanno and A. Bonardi and C. Bonavolontá and G. Bonnoli and P. Bordas and M. Böttcher and J. Bregeon and A. Brill and A.M. Brown and K. Brügge and P. Brun and P. Bruno and A. Bulgarelli and T. Bulik and M. Burton and A. Burtovoi and G. Busetto and R. Cameron and R. Canestrari and M. Capalbi and A. Caproni and R. Capuzzo-Dolcetta and P. Caraveo and S. Caroff and R. Carosi and S. Casanova and E. Cascone and F. Cassol and F. Catalani and O. Catalano and D. Cauz and M. Cerruti and S. Chaty and A. Chen and M. Chernyakova and G. Chiaro and M. Cieślar and S.M. Colak and V. Conforti and E. Congiu and J.L. Contreras and J. Cortina and A. Costa and H. Costantini and G. Cotter and P. Cristofari and P. Cumani and G. Cusumano and A. D’Aí and F. D’Ammando and L. Dangeon and P. {Da Vela} and F. Dazzi and A. {De Angelis} and V. {De Caprio} and R. {de Cássia dos Anjos} and F. {De Frondat} and E.M. {de Gouveia Dal Pino} and B. {De Lotto} and D. {De Martino} and M. {de Naurois} and E. {de Oña Wilhelmi} and F. {de Palma} and V. {de Souza} and M. {Del Santo} and C. Delgado and D. {della Volpe} and T. {Di Girolamo} and F. {Di Pierro} and L. {Di Venere} and C. Díaz and S. Diebold and A. Djannati-Ataï and A. Dmytriiev and D. {Dominis Prester} and A. Donini and D. Dorner and M. Doro and J.-L. Dournaux and J. Ebr and T.R.N. Ekoume and D. Elsässer and G. Emery and D. Falceta-Goncalves and E. Fedorova and S. Fegan and Q. Feng and G. Ferrand and E. Fiandrini and A. Fiasson and M. Filipovic and V. Fioretti and M. Fiori and S. Flis and M.V. Fonseca and G. Fontaine and L. {Freixas Coromina} and S. Fukami and Y. Fukui and S. Funk and M. Füßling and D. Gaggero and G. Galanti and R.J. {Garcia López} and M. Garczarczyk and D. Gascon and T. Gasparetto and M. Gaug and A. Ghalumyan and F. Gianotti and G. Giavitto and N. Giglietto and F. Giordano and M. Giroletti and J. Gironnet and J.-F. Glicenstein and R. Gnatyk and P. Goldoni and J.M. González and M.M. González and K.N. Gourgouliatos and T. Grabarczyk and J. Granot and D. Green and T. Greenshaw and M.-H. Grondin and O. Gueta and D. Hadasch and T. Hassan and M. Hayashida and M. Heller and O. Hervet and J. Hinton and N. Hiroshima and B. Hnatyk and W. Hofmann and P. Horvath and M. Hrabovsky and D. Hrupec and T.B. Humensky and M. Hütten and T. Inada and F. Iocco and M. Ionica and M. Iori and Y. Iwamura and M. Jamrozy and P. Janecek and D. Jankowsky and P. Jean and L. Jouvin and J. Jurysek and P. Kaaret and L.H.S. Kadowaki and S. Karkar and D. Kerszberg and B. Khélifi and D. Kieda and S. Kimeswenger and W. Kluźniak and J. Knapp and J. Knödlseder and Y. Kobayashi and B. Koch and J. Kocot and N. Komin and A. Kong and G. Kowal and M. Krause and H. Kubo and J. Kushida and P. Kushwaha and V. {La Parola} and G. {La Rosa} and M. {Lallena Arquillo} and R.G. Lang and J. Lapington and O. {Le Blanc} and J. Lefaucheur and M.A. {Leigui de Oliveira} and M. Lemoine-Goumard and J.-P. Lenain and G. Leto and R. Lico and E. Lindfors and T. Lohse and S. Lombardi and F. Longo and A. Lopez and M. López and A. Lopez-Oramas and R. López-Coto and S. Loporchio and P.L. Luque-Escamilla and E. Lyard and M.C. Maccarone and E. Mach and C. Maggio and P. Majumdar and G. Malaguti and M. Mallamaci and D. Mandat and G. Maneva and M. Manganaro and S. Mangano and M. Marculewicz and M. Mariotti and J. Martí and M. Martínez and G. Martínez and H. Martínez-Huerta and S. Masuda and N. Maxted and D. Mazin and J.-L. Meunier and M. Meyer and S. Micanovic and R. Millul and I.A. Minaya and A. Mitchell and T. Mizuno and R. Moderski and L. Mohrmann and T. Montaruli and A. Moralejo and D. Morcuende and G. Morlino and A. Morselli and E. Moulin and R. Mukherjee and P. Munar and C. Mundell and T. Murach and A. Nagai and T. Nagayoshi and T. Naito and T. Nakamori and R. Nemmen and J. Niemiec and D. Nieto and M. {Nievas Rosillo} and M. Nikołajuk and D. Ninci and K. Nishijima and K. Noda and D. Nosek and M. Nöthe and S. Nozaki and M. Ohishi and Y. Ohtani and A. Okumura and R.A. Ong and M. Orienti and R. Orito and M. Ostrowski and N. Otte and Z. Ou and I. Oya and A. Pagliaro and M. Palatiello and M. Palatka and R. Paoletti and J.M. Paredes and G. Pareschi and N. Parmiggiani and R.D. Parsons and B. Patricelli and A. Pe’er and M. Pech and P. {Peñil Del Campo} and J. Pérez-Romero and M. Perri and M. Persic and P.-O. Petrucci and O. Petruk and K. Pfrang and Q. Piel and E. Pietropaolo and M. Pohl and M. Polo and J. Poutanen and E. Prandini and N. Produit and H. Prokoph and M. Prouza and H. Przybilski and G. Pühlhofer and M. Punch and F. Queiroz and A. Quirrenbach and S. Rainò and R. Rando and S. Razzaque and O. Reimer and N. Renault-Tinacci and Y. Renier and D. Ribeiro and M. Ribó and J. Rico and F. Rieger and V. Rizi and G. {Rodriguez Fernandez} and J.C. Rodriguez-Ramirez and J.J. {Rodrí-guez Vázquez} and P. Romano and G. Romeo and M. Roncadelli and J. Rosado and G. Rowell and B. Rudak and A. Rugliancich and C. Rulten and I. Sadeh and L. Saha and T. Saito and S. Sakurai and F. {Salesa Greus} and P. Sangiorgi and H. Sano and M. Santander and A. Santangelo and R. Santos-Lima and A. Sanuy and K. Satalecka and F.G. Saturni and U. Sawangwit and S. Schlenstedt and P. Schovanek and F. Schussler and U. Schwanke and E. Sciacca and S. Scuderi and K. Sedlaczek and M. Seglar-Arroyo and O. Sergijenko and K. Seweryn and A. Shalchi and R.C. Shellard and H. Siejkowski and A. Sillanpää and A. Sinha and G. Sironi and V. Sliusar and A. Slowikowska and H. Sol and A. Specovius and S. Spencer and G. Spengler and A. Stamerra and S. Stanič and Ł. Stawarz and S. Stefanik and T. Stolarczyk and U. Straumann and T. Suomijarvi and P. Świerk and T. Szepieniec and G. Tagliaferri and H. Tajima and T. Tam and F. Tavecchio and L. Taylor and L.A. Tejedor and P. Temnikov and T. Terzic and V. Testa and L. Tibaldo and C.J. {Todero Peixoto} and F. Tokanai and L. Tomankova and D. Tonev and D.F. Torres and G. Tosti and L. Tosti and N. Tothill and F. Toussenel and G. Tovmassian and P. Travnicek and C. Trichard and G. Umana and V. Vagelli and M. Valentino and B. Vallage and P. Vallania and L. Valore and J. Vandenbroucke and G.S. Varner and G. Vasileiadis and V. Vassiliev and M. {Vázquez Acosta} and M. Vecchi and S. Vercellone and S. Vergani and G.P. Vettolani and A. Viana and C.F. Vigorito and J. Vink and V. Vitale and H. Voelk and A. Vollhardt and S. Vorobiov and S.J. Wagner and R. Walter and F. Werner and R. White and A. Wierzcholska and M. Will and D.A. Williams and R. Wischnewski and L. Yang and T. Yoshida and T. Yoshikoshi and M. Zacharias and L. Zampieri and M. Zavrtanik and D. Zavrtanik and A.A. Zdziarski and A. Zech and H. Zechlin and A. Zenin and V.I. Zhdanov and S. Zimmer and J. Zorn},
keywords = {Monte Carlo simulations, Cherenkov telescopes, IACT technique, Gamma rays, Cosmic rays},
abstract = {The Cherenkov Telescope Array (CTA) is the major next-generation observatory for ground-based very-high-energy gamma-ray astronomy. It will improve the sensitivity of current ground-based instruments by a factor of five to twenty, depending on the energy, greatly improving both their angular and energy resolutions over four decades in energy (from 20 GeV to 300 TeV). This achievement will be possible by using tens of imaging Cherenkov telescopes of three successive sizes. They will be arranged into two arrays, one per hemisphere, located on the La Palma island (Spain) and in Paranal (Chile). We present here the optimised and final telescope arrays for both CTA sites, as well as their foreseen performance, resulting from the analysis of three different large-scale Monte Carlo productions.}
}

@article{cta_australia, title={Performance of a small array of Imaging Air Cherenkov Telescopes sited in Australia}, volume={39}, DOI={10.1017/pasa.2022.29}, journal={Publications of the Astronomical Society of Australia}, author={Lee, Simon and Einecke, Sabrina and Rowell, Gavin and Balazs, Csaba and Bellido, Jose A. and Dai, Shi and Elsässer, Dominik and Filipović, Miroslav and Harvey, Violet M. and McGee, Padric and et al.}, year={2022}, pages={e041}}


@software{lstchain,
  author       = {Ruben Lopez-Coto and
                  Thomas Vuillaume and
                  Abelardo Moralejo and
                  Franca Cassol and
                  Maximilian Nöthe and
                  Daniel Morcuende and
                  Chaitanya Priyadarshi and
                  Mab Bernardos and
                  Seiya Nozaki and
                  Paweł Gliwny and
                  Jose Enrique Ruiz and
                  Enrique Garcia and
                  Mykhailo Dalchenko and
                  yrenier and
                  Lab Saha and
                  Mikaël Jacquemont and
                  Dominik Neise and
                  Cyril Alispach and
                  Roberta Pillera and
                  Andres-Baquero and
                  Julian Sitarek and
                  aaguasca and
                  Mari Takahashi and
                  sn621 and
                  yiwamura},
  title        = {cta-observatory/cta-lstchain: v0.9.4},
  month        = mar,
  year         = 2022,
  publisher    = {Zenodo},
  version      = {v0.9.4},
  doi          = {10.5281/zenodo.6344674},
  url          = {https://doi.org/10.5281/zenodo.6344674},
}


@Article{gadf,
AUTHOR = {Nigro, Cosimo and Hassan, Tarek and Olivera-Nieto, Laura},
TITLE = {Evolution of Data Formats in Very-High-Energy Gamma-Ray Astronomy},
JOURNAL = {Universe},
VOLUME = {7},
YEAR = {2021},
NUMBER = {10},
ARTICLE-NUMBER = {374},
URL = {https://www.mdpi.com/2218-1997/7/10/374},
ISSN = {2218-1997},
ABSTRACT = {Most major scientific results produced by ground-based gamma-ray telescopes in the last 30 years have been obtained by expert members of the collaborations operating these instruments. This is due to the proprietary data and software policies adopted by these collaborations. However, the advent of the next generation of telescopes and their operation as observatories open to the astronomical community, along with a generally increasing demand for open science, confront gamma-ray astronomers with the challenge of sharing their data and analysis tools. As a consequence, in the last few years, the development of open-source science tools has progressed in parallel with the endeavour to define a standardised data format for astronomical gamma-ray data. The latter constitutes the main topic of this review. Common data specifications provide equally important benefits to the current and future generation of gamma-ray instruments: they allow the data from different instruments, including legacy data from decommissioned telescopes, to be easily combined and analysed within the same software framework. In addition, standardised data accessible to the public, and analysable with open-source software, grant fully-reproducible results. In this article, we provide an overview of the evolution of the data format for gamma-ray astronomical data, focusing on its progression from private and diverse specifications to prototypical open and standardised ones. The latter have already been successfully employed in a number of publications paving the way to the analysis of data from the next generation of gamma-ray instruments, and to an open and reproducible way of conducting gamma-ray astronomy.},
DOI = {10.3390/universe7100374}
}

@software{gammapy,
  author       = {Axel Donath and
                  Christoph Deil and
                  Régis Terrier and
                  Johannes King and
                  Jose Enrique Ruiz and
                  Quentin Remy and
                  Léa Jouvin and
                  Atreyee Sinha and
                  Matthew Wood and
                  Fabio Pintore and
                  Manuel Paz Arribas and
                  Laura Olivera and
                  Luca Giunti and
                  Bruno Khelifi and
                  Ellis Owen and
                  Brigitta Sipőcz and
                  Olga Vorokh and
                  Julien Lefaucheur and
                  Fabio Acero and
                  Thomas Robitaille and
                  David Fidalgo and
                  Jonathan D. Harris and
                  Lars Mohrmann and
                  Cosimo Nigro and
                  Dirk Lennarz and
                  Jaleled Eddine Hajlaoui and
                  Alexis de Almeida Coutinho and
                  Matthias Wegenmat and
                  Dimitri Papadopoulos and
                  Maximilian Nöthe and
                  Nachiketa Chakraborty and
                  Michael Droettboom and
                  Jason Watson and
                  Helen Poon and
                  Arjun Voruganti and
                  Vikas Joshi and
                  Thomas Armstrong and
                  Erik Tollerud and
                  Erik M. Bray and
                  Domenico Tiziani and
                  Gabriel Emery and
                  Hubert Siejkowski and
                  Kai Brügge and
                  Luigi Tibaldo and
                  Arpit Gogia and
                  Ignacio Minaya and
                  Marion Spir-Jacob and
                  Yves Gallant and
                  Andrew W. Chen and
                  Roberta Zanin and
                  Jean-Philippe Lenain and
                  Larry Bradley and
                  Kaori Nakashima and
                  Anne Lemière and
                  Mathieu de Bony and
                  Matthew Craig and
                  Lab Saha and
                  Zé Vinicius and
                  Kyle Barbary and
                  Thomas Vuillaume and
                  Daniel Morcuende and
                  José Luis Contreras and
                  Laura Vega García and
                  Oscar Blanch Bigas and
                  Víctor Zabalza and
                  Wolfgang Kerzendorf and
                  Rolf Buehler and
                  Sebastian Panny and
                  Silvia Manconi and
                  Stefan Klepser and
                  Peter Deiml and
                  Johanes Buchner and
                  Hugo van Kemenade and
                  Eriuc O. Lebigot and
                  Benjamin Alan Weaver and
                  Debanjan Bose and
                  Rubén López-Coto and
                  Sam Carter},
  title        = {gammapy/gammapy: v.0.19},
  month        = nov,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {v0.19},
  doi          = {10.5281/zenodo.5721467},
  url          = {https://doi.org/10.5281/zenodo.5721467},
}


@article{sensitivity_a,
doi = {10.3847/1538-4357/ace89d},
url = {https://dx.doi.org/10.3847/1538-4357/ace89d},
year = {2023},
month = {oct},
publisher = {The American Astronomical Society},
volume = {956},
number = {2},
pages = {80},
author = {Abe, H. and Abe, K. and Abe, S. and Aguasca-Cabot, A. and Agudo, I. and Alvarez Crespo, N. and Antonelli, L. A. and Aramo, C. and Arbet-Engels, A. and Arcaro, C. and Artero, M. and Asano, K. and Aubert, P. and Baktash, A. and Bamba, A. and Baquero Larriva, A. and Baroncelli, L. and Barres de Almeida, U. and Barrio, J. A. and Batkovic, I. and Baxter, J. and Becerra González, J. and Bernardini, E. and Bernardos, M. I. and Bernete Medrano, J. and Berti, A. and Bhattacharjee, P. and Biederbeck, N. and Bigongiari, C. and Bissaldi, E. and Blanch, O. and Bonnoli, G. and Bordas, P. and Borghese, A. and Bulgarelli, A. and Burelli, I. and Buscemi, M. and Cardillo, M. and Caroff, S. and Carosi, A. and Cassol, F. and Cauz, D. and Ceribella, G. and Chai, Y. and Cheng, K. and Chiavassa, A. and Chikawa, M. and Chytka, L. and Cifuentes, A. and Contreras, J. L. and Cortina, J. and Costantini, H. and D’Amico, G. and Dalchenko, M. and De Angelis, A. and de Bony de Lavergne, M. and De Lotto, B. and de Menezes, R. and Deleglise, G. and Delgado, C. and Delgado Mengual, J. and della Volpe, D. and Dellaiera, M. and Depaoli, D. and Di Piano, A. and Di Pierro, F. and Di Tria, R. and Di Venere, L. and Díaz, C. and Dominik, R. M. and Dominis Prester, D. and Donini, A. and Dorner, D. and Doro, M. and Elsässer, D. and Emery, G. and Escudero, J. and Fallah Ramazani, V. and Ferrara, G. and Ferrarotto, F. and Fiasson, A. and Freixas Coromina, L. and Fröse, S. and Fukami, S. and Fukazawa, Y. and Garcia, E. and Garcia López, R. and Gasbarra, C. and Gasparrini, D. and Geyer, F. and Giesbrecht Paiva, J. and Giglietto, N. and Giordano, F. and Giro, E. and Gliwny, P. and Godinovic, N. and Grau, R. and Green, D. and Green, J. and Gunji, S. and Hackfeld, J. and Hadasch, D. and Hahn, A. and Hashiyama, K. and Hassan, T. and Hayashi, K. and Heckmann, L. and Heller, M. and Herrera Llorente, J. and Hirotani, K. and Hoffmann, D. and Horns, D. and Houles, J. and Hrabovsky, M. and Hrupec, D. and Hui, D. and Hütten, M. and Iarlori, M. and Imazawa, R. and Inada, T. and Inome, Y. and Ioka, K. and Iori, M. and Ishio, K. and Iwamura, Y. and Jacquemont, M. and Jimenez Martinez, I. and Jurysek, J. and Kagaya, M. and Karas, V. and Katagiri, H. and Kataoka, J. and Kerszberg, D. and Kobayashi, Y. and Kong, A. and Kubo, H. and Kushida, J. and Lainez, M. and Lamanna, G. and Lamastra, A. and Le Flour, T. and Linhoff, M. and Longo, F. and López-Coto, R. and López-Moya, M. and López-Oramas, A. and Loporchio, S. and Lorini, A. and Luque-Escamilla, P. L. and Majumdar, P. and Makariev, M. and Mandat, D. and Manganaro, M. and Manicò, G. and Mannheim, K. and Mariotti, M. and Marquez, P. and Marsella, G. and Martí, J. and Martinez, O. and Martínez, G. and Martínez, M. and Marusevec, P. and Mas-Aguilar, A. and Maurin, G. and Mazin, D. and Mestre Guillen, E. and Micanovic, S. and Miceli, D. and Miener, T. and Miranda, J. M. and Mirzoyan, R. and Mizuno, T. and Molero Gonzalez, M. and Molina, E. and Montaruli, T. and Monteiro, I. and Moralejo, A. and Morcuende, D. and Morselli, A. and Mrakovcic, K. and Murase, K. and Nagai, A. and Nagataki, S. and Nakamori, T. and Nickel, L. and Nievas, M. and Nishijima, K. and Noda, K. and Nosek, D. and Nozaki, S. and Ohishi, M. and Ohtani, Y. and Oka, T. and Okazaki, N. and Okumura, A. and Orito, R. and Otero-Santos, J. and Palatiello, M. and Paneque, D. and Pantaleo, F. R. and Paoletti, R. and Paredes, J. M. and Pech, M. and Pecimotika, M. and Peresano, M. and Pérez, A. and Pietropaolo, E. and Pirola, G. and Plard, C. and Podobnik, F. and Poireau, V. and Polo, M. and Pons, E. and Prandini, E. and Prast, J. and Principe, G. and Priyadarshi, C. and Prouza, M. and Rando, R. and Rhode, W. and Ribó, M. and Rizi, V. and Rodriguez Fernandez, G. and Ruiz, J. E. and Saito, T. and Sakurai, S. and Sanchez, D. A. and Šarić, T. and Sato, Y. and Saturni, F. G. and Schleicher, B. and Schmuckermaier, F. and Schubert, J. L. and Schussler, F. and Schweizer, T. and Seglar Arroyo, M. and Silvia, R. and Sitarek, J. and Sliusar, V. and Spolon, A. and Strišković, J. and Strzys, M. and Suda, Y. and Sunada, Y. and Tajima, H. and Takahashi, H. and Takahashi, M. and Takata, J. and Takeishi, R. and Tam, P. H. T. and Tanaka, S. J. and Tateishi, D. and Tejedor, L. A. and Temnikov, P. and Terada, Y. and Terauchi, K. and Terzic, T. and Teshima, M. and Tluczykont, M. and Tokanai, F. and Torres, D. F. and Travnicek, P. and Truzzi, S. and Tutone, A. and Uhlrich, G. and Vacula, M. and Vallania, P. and van Scherpenberg, J. and Vázquez Acosta, M. and Verguilov, V. and Viale, I. and Vigliano, A. and Vigorito, C. F. and Vitale, V. and Voutsinas, G. and Vovk, I. and Vuillaume, T. and Walter, R. and Will, M. and Yamamoto, T. and Yamazaki, R. and Yoshida, T. and Yoshikoshi, T. and Zywucka, N. and Bernlöhr, K. and Gueta, O. and Kosack, K. and Maier, G. and Watson, J.},
title = {Observations of the Crab Nebula and Pulsar with the Large-sized Telescope Prototype of the Cherenkov Telescope Array},
journal = {The Astrophysical Journal},
abstract = {The Cherenkov Telescope Array (CTA) is a next-generation ground-based observatory for gamma-ray astronomy at very high energies. The Large-Sized Telescope prototype (LST-1) is located at the CTA-North site, on the Canary Island of La Palma. LSTs are designed to provide optimal performance in the lowest part of the energy range covered by CTA, down to ≃20 GeV. LST-1 started performing astronomical observations in 2019 November, during its commissioning phase, and it has been taking data ever since. We present the first LST-1 observations of the Crab Nebula, the standard candle of very-high-energy gamma-ray astronomy, and use them, together with simulations, to assess the performance of the telescope. LST-1 has reached the expected performance during its commissioning period—only a minor adjustment of the preexisting simulations was needed to match the telescope’s behavior. The energy threshold at trigger level is around 20 GeV, rising to ≃30 GeV after data analysis. Performance parameters depend strongly on energy, and on the strength of the gamma-ray selection cuts in the analysis: angular resolution ranges from 0.°12–0.°40, and energy resolution from 15%–50%. Flux sensitivity is around 1.1% of the Crab Nebula flux above 250 GeV for a 50 hr observation (12% for 30 minutes). The spectral energy distribution (in the 0.03–30 TeV range) and the light curve obtained for the Crab Nebula agree with previous measurements, considering statistical and systematic uncertainties. A clear periodic signal is also detected from the pulsar at the center of the Nebula.}
}


@article{sensitivity_b,
	author = {{Abe, H.} and {Abe, K.} and {Abe, S.} and {Acciari, V. A.} and {Aguasca-Cabot, A.} and {Agudo, I.} and {Alvarez Crespo, N.} and {Aniello, T.} and {Ansoldi, S.} and {Antonelli, L. A.} and {Aramo, C.} and {Arbet-Engels, A.} and {Arcaro, C.} and {Artero, M.} and {Asano, K.} and {Aubert, P.} and {Baack, D.} and {Babić, A.} and {Baktash, A.} and {Bamba, A.} and {Baquero Larriva, A.} and {Baroncelli, L.} and {Barres de Almeida, U.} and {Barrio, J. A.} and {Batković, I.} and {Baxter, J.} and {Becerra González, J.} and {Bednarek, W.} and {Bernardini, E.} and {Bernardos, M. I.} and {Bernete Medrano, J.} and {Berti, A.} and {Besenrieder, J.} and {Bhattacharjee, P.} and {Biederbeck, N.} and {Bigongiari, C.} and {Biland, A.} and {Bissaldi, E.} and {Blanch, O.} and {Bonnoli, G.} and {Bordas, P.} and {Bošnjak, Ž.} and {Bulgarelli, A.} and {Burelli, I.} and {Burmistrov, L.} and {Buscemi, M.} and {Busetto, G.} and {Campoy Ordaz, A.} and {Cardillo, M.} and {Caroff, S.} and {Carosi, A.} and {Carosi, R.} and {Carrasco, M. S.} and {Carretero-Castrillo, M.} and {Cassol, F.} and {Castro-Tirado, A. J.} and {Cauz, D.} and {Cerasole, D.} and {Ceribella, G.} and {Chai, Y.} and {Cheng, K.} and {Chiavassa, A.} and {Chikawa, M.} and {Chytka, L.} and {Cifuentes, A.} and {Cikota, S.} and {Colombo, E.} and {Contreras, J. L.} and {Cornelia, A.} and {Cortina, J.} and {Costantini, H.} and {Covino, S.} and {D’Amico, G.} and {D’Elia, V.} and {Da Vela, P.} and {Dalchenko, M.} and {Dazzi, F.} and {De Angelis, A.} and {de Bony de Lavergne, M.} and {De Lotto, B.} and {De Lucia, M.} and {de Menezes, R.} and {Del Peral, L.} and {Del Popolo, A.} and {Deleglise, G.} and {Delfino, M.} and {Delgado Mendez, C.} and {Delgado Mengual, J.} and {della Volpe, D.} and {Dellaiera, M.} and {Depaoli, D.} and {De Angelis, A.} and {Di Piano, A.} and {Di Pierro, F.} and {Di Pilato, A.} and {Di Tria, R.} and {Di Venere, L.} and {Dominik, R. M.} and {Dominis Prester, D.} and {Donini, A.} and {Dorner, D.} and {Doro, M.} and {Díaz, C.} and {Eisenberger, L.} and {Elsässer, D.} and {Emery, G.} and {Escudero, J.} and {Fallah Ramazani, V.} and {Fariña, L.} and {Fattorini, A.} and {Ferrara, G.} and {Ferrarotto, F.} and {Fiasson, A.} and {Foffano, L.} and {Font, L.} and {Freixas Coromina, L.} and {Fröse, S.} and {Fukami, S.} and {Fukazawa, Y.} and {Garcia López, R. J.} and {Garcia, E.} and {Garczarczyk, M.} and {García López, R. J.} and {Gasbarra, C.} and {Gasparrini, D.} and {Gasparyan, S.} and {Gaug, M.} and {Geyer, D.} and {Giesbrecht Paiva, J. G.} and {Giglietto, N.} and {Giordano, F.} and {Gliwny, P.} and {Godinović, N.} and {Grau, R.} and {Green, D.} and {Green, J. G.} and {Gunji, S.} and {Günther, P.} and {Hackfeld, J.} and {Hadasch, D.} and {Hahn, A.} and {Hashiyama, K.} and {Hassan, T.} and {Hayashi, K.} and {Heckmann, L.} and {Heller, M.} and {Herrera Llorente, J.} and {Hirotani, K.} and {Hoffmann, D.} and {Horns, D.} and {Houles, J.} and {Hrabovsky, M.} and {Hrupec, D.} and {Hui, D.} and {Hütten, M.} and {Iarlori, M.} and {Imazawa, R.} and {Inada, T.} and {Inome, Y.} and {Ioka, K.} and {Iori, M.} and {Iotov, R.} and {Ishio, K.} and {Jacquemont, M.} and {Jiménez Martínez, I.} and {Jobst, E.} and {Jormanainen, J.} and {Jurysek, J.} and {Kagaya, M.} and {Karas, V.} and {Katagiri, H.} and {Kataoka, J.} and {Kerszberg, D.} and {Kluge, G. W.} and {Kobayashi, Y.} and {Kohri, K.} and {Kong, A.} and {Kouch, P. M.} and {Kubo, H.} and {Kushida, J.} and {Lainez, M.} and {Lamanna, G.} and {Lamastra, A.} and {Le Flour, T.} and {Leone, F.} and {Lindfors, E.} and {Linhoff, L.} and {Linhoff, M.} and {Lombardi, S.} and {Longo, F.} and {Loporchio, S.} and {Lorini, A.} and {Lozano Bahilo, J.} and {Luque-Escamilla, P. L.} and {Lyard, E.} and {Láinez Lezáun, M.} and {López-Coto, R.} and {López-Moya, M.} and {López-Oramas, A.} and {Machado de Oliveira Fraga, B.} and {Majumdar, P.} and {Makariev, M.} and {Mandat, D.} and {Maneva, G.} and {Manganaro, M.} and {Mangano, S.} and {Mang, N.} and {Manicò, G.} and {Mannheim, K.} and {Mariotti, M.} and {Marquez, P.} and {Marsella, G.} and {Martinez, O.} and {Martínez, G.} and {Martínez, M.} and {Martí, J.} and {Mas-Aguilar, A.} and {Maurin, G.} and {Mazin, D.} and {Menchiari, S.} and {Mender, S.} and {Mestre Guillen, E.} and {Micanovic, S.} and {Miceli, D.} and {Miener, T.} and {Miranda, J. M.} and {Mirzoyan, R.} and {Mizuno, T.} and {Mićanović, S.} and {Molero González, M.} and {Molina, E.} and {Mondal, H. A.} and {Montaruli, T.} and {Monteiro, I.} and {Moralejo, A.} and {Morcuende, D.} and {Morselli, A.} and {Moya, V.} and {Muraishi, H.} and {Murase, K.} and {Nagataki, S.} and {Nakamori, T.} and {Nanci, C.} and {Neronov, A.} and {Neustroev, V.} and {Nickel, L.} and {Nievas Rosillo, M.} and {Nigro, C.} and {Nikolić, L.} and {Nilsson, K.} and {Nishijima, K.} and {Njoh Ekoume, T.} and {Noda, K.} and {Nosek, D.} and {Nozaki, S.} and {Ohishi, M.} and {Ohtani, Y.} and {Oka, T.} and {Okumura, A.} and {Orito, R.} and {Otero-Santos, J.} and {Paiano, S.} and {Palatiello, M.} and {Paneque, D.} and {Pantaleo, F. R.} and {Paoletti, R.} and {Paredes, J. M.} and {Pavletić, L.} and {Pech, M.} and {Pecimotika, M.} and {Peresano, M.} and {Persic, M.} and {Pfeiffle, F.} and {Pietropaolo, E.} and {Pihet, M.} and {Pirola, G.} and {Plard, C.} and {Podobnik, F.} and {Poireau, V.} and {Polo, M.} and {Pons, E.} and {Prada Moroni, P. G.} and {Prandini, E.} and {Prast, J.} and {Principe, G.} and {Priyadarshi, C.} and {Prouza, M.} and {Rando, R.} and {Rhode, W.} and {Ribó, M.} and {Rico, J.} and {Righi, C.} and {Rizi, V.} and {Rodriguez Fernandez, G.} and {Rodríguez Frías, M. D.} and {Sahakyan, N.} and {Saito, T.} and {Sakurai, S.} and {Sanchez, D. A.} and {Satalecka, K.} and {Sato, M.} and {Sato, Y.} and {Saturni, F. G.} and {Savchenko, V.} and {Schleicher, B.} and {Schmidt, K.} and {Schmuckermaier, F.} and {Schubert, J. L.} and {Schussler, F.} and {Schweizer, T.} and {Sciaccaluga, A.} and {Siegert, T.} and {Silvia, R.} and {Sitarek, J.} and {Sliusar, V.} and {Sobczynska, D.} and {Spolon, A.} and {Stamerra, A.} and {Strišković, J.} and {Strom, D.} and {Strzys, M.} and {Suda, Y.} and {Suutarinen, S.} and {Šarić, T.} and {Tajima, H.} and {Takahashi, H.} and {Takahashi, M.} and {Takata, J.} and {Takeishi, R.} and {Tam, P. H. T.} and {Tanaka, S. J.} and {Tateishi, D.} and {Tavecchio, F.} and {Temnikov, P.} and {Terada, Y.} and {Terauchi, K.} and {Terzić, T.} and {Teshima, M.} and {Tluczykont, M.} and {Tokanai, F.} and {Torres, D. F.} and {Tosti, L.} and {Travnicek, P.} and {Truzzi, S.} and {Tutone, A.} and {Ubach, S.} and {Vacula, M.} and {Vallania, P.} and {van Scherpenberg, J.} and {Vazquez Acosta, M.} and {Ventura, S.} and {Verguilov, V.} and {Viale, I.} and {Vigliano, A.} and {Vigorito, C. F.} and {Visentin, E.} and {Vitale, V.} and {Voutsinas, G.} and {Vovk, I.} and {Vuillaume, T.} and {Vázquez Acosta, M.} and {Walter, R.} and {Wei, Z.} and {Will, M.} and {Yamamoto, T.} and {Yamazaki, R.} and {Yoshida, T.} and {Yoshikoshi, T.} and {Zywucka, N.}},
	title = {Performance of the joint LST-1 and MAGIC observations evaluated with Crab Nebula data},
	DOI= "10.1051/0004-6361/202346927",
	url= "https://doi.org/10.1051/0004-6361/202346927",
	journal = {A&A},
	year = 2023,
	volume = 680,
	pages = "A66",
}

@article{cta_config_b,
title = {Monte Carlo design studies for the Cherenkov Telescope Array},
journal = {Astroparticle Physics},
volume = {43},
pages = {171-188},
year = {2013},
note = {Seeing the High-Energy Universe with the Cherenkov Telescope Array - The Science Explored with the CTA},
issn = {0927-6505},
doi = {https://doi.org/10.1016/j.astropartphys.2012.10.002},
url = {https://www.sciencedirect.com/science/article/pii/S0927650512001867},
author = {K. Bernlöhr and A. Barnacka and Y. Becherini and O. {Blanch Bigas} and E. Carmona and P. Colin and G. Decerprit and F. {Di Pierro} and F. Dubois and C. Farnier and S. Funk and G. Hermann and J.A. Hinton and T.B. Humensky and B. Khélifi and T. Kihm and N. Komin and J.-P. Lenain and G. Maier and D. Mazin and M.C. Medina and A. Moralejo and S.J. Nolan and S. Ohm and E. {de Oña Wilhelmi} and R.D. Parsons and M. {Paz Arribas} and G. Pedaletti and S. Pita and H. Prokoph and C.B. Rulten and U. Schwanke and M. Shayduk and V. Stamatescu and P. Vallania and S. Vorobiov and R. Wischnewski and T. Yoshikoshi and A. Zech},
keywords = {Monte Carlo simulations, Cherenkov telescopes, IACT technique, Gamma rays, Cosmic rays},
abstract = {The Cherenkov Telescopes Array (CTA) is planned as the future instrument for very-high-energy (VHE) gamma-ray astronomy with a wide energy range of four orders of magnitude and an improvement in sensitivity compared to current instruments of about an order of magnitude. Monte Carlo simulations are a crucial tool in the design of CTA. The ultimate goal of these simulations is to find the most cost-effective solution for given physics goals and thus sensitivity goals or to find, for a given cost, the solution best suited for different types of targets with CTA. Apart from uncertain component cost estimates, the main problem in this procedure is the dependence on a huge number of configuration parameters, both in specifications of individual telescope types and in the array layout. This is addressed by simulation of a huge array intended as a superset of many different realistic array layouts, and also by simulation of array subsets for different telescope parameters. Different analysis methods – in use with current installations and extended (or developed specifically) for CTA – are applied to the simulated data sets for deriving the expected sensitivity of CTA. In this paper we describe the current status of this iterative approach to optimize the CTA design and layout.}
}
